Supporting Schema References in Keyword Queries over Relational Databases

Relational Keyword Search (R-KwS) systems enable naive/informal users to explore and retrieve information from relational databases without knowing schema details or query languages. These systems take the keywords from the input query, locate the elements of the target database that correspond to these keywords, and look for ways to "connect" these elements using information on referential integrity constraints, i.e., key/foreign key pairs. Although several such systems have been proposed in the literature, most of them only support queries whose keywords refer to the contents of the target database and just very few support queries in which keywords refer to elements of the database schema. This paper proposes LATHE, a novel R-KwS designed to support such queries. To this end, in our work, we first generalize the well-known concepts of Query Matches (QMs) and Candidate Joining Networks (CJNs) to handle keywords referring to schema elements and propose new algorithms to generate them. Then, we introduce an approach to automatically select the CJNs that are more likely to represent the user intent when issuing a keyword query. This approach includes two major innovations: a ranking algorithm for selecting better QMs, yielding the generation of fewer but better CJNs, and an eager evaluation strategy for pruning void useless CJNs. We present a comprehensive set of experiments performed with query sets and datasets previously used in experiments with state-of-the-art R-KwS systems and methods. Our results indicate that LATHE can handle a wider variety of keyword queries while remaining highly effective, even for large databases with intricate schemas.

==> tables/tab_SQL_listing1.tex <==
\begin{lstlisting}
SELECT m.title, p.name
FROM person p
JOIN casting c ON  p.id=c.pid
JOIN movie m ON m.id = c.mid
WHERE p.name ILIKE '%will%' 
AND p.name ILIKE '%smith%';
\end{lstlisting} 

==> tables/tab_SQL_listing2.tex <==
\begin{lstlisting}
	SELECT m.title, p1.name, p2.name
	FROM person p1
	JOIN casting c1 ON p1.id=c1.pid
	JOIN movie m ON m.id = c1.mid
	JOIN casting c2 ON m.id = c2.mid
	JOIN person p2 ON p2.id=c2.pid
	WHERE p1.name ILIKE '%will%' 
	AND p2.name ILIKE '%smith%'
	AND p1.id<>p2.id;
\end{lstlisting}
